Self-Serviced IoT: Practical and Private IoT Computation Offloading with Full User Control

The rapid increase in the adoption of Internet-of-Things (IoT) devices raises critical privacy concerns as these devices can access a variety of sensitive data. The current status quo of relying on manufacturers' cloud services to process this data is especially problematic since users cede control once their data leaves their home. Multiple recent incidents further call into question if vendors can indeed be trusted with users' data. At the same time, users desire compelling features supported by IoT devices and ML-based cloud inferences which compels them to subscribe to manufacturer-managed cloud services. An alternative to use a local in-home hub requires substantial hardware investment, management, and scalability limitations. This paper proposes Self-Serviced IoT (SSIoT), a clean-slate approach of using a hybrid hub-cloud setup to enable privacy-aware computation offload for IoT applications. Uniquely, SSIoT enables opportunistic computation offload to public cloud providers while still ensuring that the end-user retains complete end-to-end control of their private data reducing the trust required from public cloud providers. We show that SSIoT can leverage emerging function-as-a-service computation (e.g. AWS Lambda) to make these offloads cost-efficient, scalable and high performance as long as key limitations of being stateless, limited resources, and security isolation can be addressed. We build an end-to-end prototype of SSIoT and evaluate it using several micro-benchmarks and example applications representing real-world IoT use cases. Our results show that SSIoT is highly scalable, as compared to local-only approaches which struggle with as little as 2-4 apps in parallel. We also show that SSIoT is cost-efficient (operating a smart doorbell for $10 a year) at the cost of minimal additional latency as compared to a local-only hub, even with a hardware ML accelerator.

==> tikz-plots/kms-messages.tex <==
\begin{tikzpicture}[every node/.style={font=\footnotesize, inner sep=2pt, fill=none, 
		text=black, align=center}]
	
	\node[draw] (hub) at (0pt,0pt) {\SSIoT Hub \\ ($K_A, K_A^{-1}, K_M, K$)};
	\node[above=0pt of hub] (hub-icon) {\includegraphics[width=15pt]{figures/router.png}};
	
	
	\node[right=120pt of hub, draw] (app) {FaaS App\\Instance\\($K_A$)};
	\node[right=0pt of app] (app-icon) {\includegraphics[width=15pt]{figures/web-programming.png}};
	
	\path[thick, draw, -{latex}] (hub) -- node [midway, above] {$m_1 :=$ \encryptedDataFile} (app);
	\path[thick, draw, -{latex}] (hub) -- node [midway, below] {$m_2 :=$ \encryptedDataKey} (app);
		
	\node[above=30pt of app, draw] (kms) {\SSIoT KMS\\($K_M, K_M^{-1}, K_A$)};
	\node[left=0pt of kms] (kms-icon) {\includegraphics[width=15pt]{figures/servers.png}};
	
	
	\path[thick, draw, -{latex},  transform canvas={xshift=-0.25em}] (app) -- node [text width=2cm, midway,  transform canvas={xshift=-0.75em}] {$m_2$} (kms);
	\path[thick, draw, -{latex},  transform canvas={xshift=0.25em}] (kms) -- node [text width=2cm, midway,  transform canvas={xshift=0.75em}] {$K$} (app);
	
	
\end{tikzpicture}

==> tikz-plots/ssiot-deployment.tex <==
\begin{tikzpicture}[every node/.style={font=\footnotesize, inner sep=2pt, fill=none, 
    text=black, align=center}]
	
	\node[draw] (hub) at (0pt,0pt) {\SSIoT \\ Hub};
	\node[left=0pt of hub] (hub-icon) {\includegraphics[width=15pt]{figures/router.png}};
	
	\node[above right=20pt and 60pt of hub, draw] (kms) {\SSIoT \\ KMS};
	\node[right=0pt of kms] (kms-icon) {\includegraphics[width=15pt]{figures/servers.png}};
	
	\node[right=100pt of hub, draw] (faas) {FaaS \\ Platform};
	\node[above right=-20pt and 0pt of faas] (faas-icon) {\includegraphics[width=25pt]{figures/lambda.png}};
	
	
	\path[thick, draw, -{latex}] (hub) -- node [text width=2cm,midway,above, align=left ] (step-1-text) {Register App Public Key}  (kms);
	\node[left=0pt of step-1-text] (step-1) {\circled{1}};
	
	\path[thick, draw, -{latex}] (hub) -- node [text width=5cm, midway, above ] {\circled{2} Upload App Package} (faas);
	
\end{tikzpicture}

==> tikz-plots/ssiot-invocation.tex <==
\begin{tikzpicture}[every node/.style={font=\footnotesize, inner sep=2pt, fill=none, 
		text=black, align=center}]
	
	\node[draw] (hub) at (0pt,0pt) {\SSIoT \\ Hub};
	\node[above=0pt of hub] (hub-icon) {\includegraphics[width=15pt]{figures/router.png}};
	
	
	\node[left=20pt of hub] (device) {\includegraphics[width=15pt]{figures/video-camera.png}\\Device};
	
	\path[thick, draw, -{latex}] (device) -- node [text width=2cm,midway,above] {\circled{1}} (hub);
	
	\node[right=25pt of hub, draw] (faas) {FaaS \\ Platform};
	\node[above=0pt of faas] (faas-icon) {\includegraphics[width=25pt]{figures/lambda.png}};
	

	\path[thick, draw, -{latex}] (hub) -- node [text width=2cm, midway, above] {\circled{2}} (faas);

	
	\node[right=25pt of faas, draw] (app) {FaaS App\\Instance};
	\node[right=0pt of app] (app-icon) {\includegraphics[width=15pt]{figures/web-programming.png}};
	
	\path[thick, draw, -{latex}] (faas) -- node [text width=2cm, midway, above] {\circled{3}} (app);
	
	\node[above=30pt of app, draw] (kms) {\SSIoT \\ KMS};
	\node[right=0pt of kms] (kms-icon) {\includegraphics[width=15pt]{figures/servers.png}};
	
	
	\path[thick, draw, -{latex},  transform canvas={xshift=-0.25em}] (app) -- node [text width=2cm, midway,  transform canvas={xshift=-0.65em}] {\circled{4}} (kms);
	\path[thick, draw, -{latex},  transform canvas={xshift=0.25em}] (kms) -- node [text width=2cm, midway,  transform canvas={xshift=0.65em}] {\circled{5}} (app);
	
	
	\coordinate[below=15pt of app]  (c1) ;
	\draw[thick] (app) -- (c1);
	\path[thick, draw, -{latex}] (c1) -| node [near start, above=0pt] {\circled{6}} (hub);
	
	
\end{tikzpicture}
